Detect Everything with Few Examples

Few-shot object detection aims at detecting novel categories given only a few example images. It is a basic skill for a robot to perform tasks in open environments. Recent methods focus on finetuning strategies, with complicated procedures that prohibit a wider application. In this paper, we introduce DE-ViT, a few-shot object detector without the need for finetuning. DE-ViT's novel architecture is based on a new region-propagation mechanism for localization. The propagated region masks are transformed into bounding boxes through a learnable spatial integral layer. Instead of training prototype classifiers, we propose to use prototypes to project ViT features into a subspace that is robust to overfitting on base classes. We evaluate DE-ViT on few-shot, and one-shot object detection benchmarks with Pascal VOC, COCO, and LVIS. DE-ViT establishes new state-of-the-art results on all benchmarks. Notably, for COCO, DE-ViT surpasses the few-shot SoTA by 15 mAP on 10-shot and 7.2 mAP on 30-shot and one-shot SoTA by 2.8 AP50. For LVIS, DE-ViT outperforms few-shot SoTA by 17 box APr. Further, we evaluate DE-ViT with a real robot by building a pick-and-place system for sorting novel objects based on example images. The videos of our robot demonstrations, the source code and the models of DE-ViT can be found at https://mlzxy.github.io/devit.

==> backup/backup.iclr2024/0.preamble.tex <==
% \usepackage[pdftex]{graphicx}
% \usepackage{lipsum}

\usepackage{comment}
\usepackage{pifont}
\usepackage{svg}
\usepackage{xcolor}
\usepackage{stackengine}

% \newcommand{\ie}{\emph{i.e.}}
% \newcommand{\eg}{\emph{e.g.}}

\newcommand{\solidone}{\ding{182}}
\newcommand{\solidtwo}{\ding{183}}
\newcommand{\solidthree}{\ding{184}}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\definecolor{lightergray}{RGB}{242, 242, 242}
\definecolor{tablegray}{RGB}{192, 192, 192}
\newcommand{\mcell}[1]{\begin{tabular}{@{}c@{}}#1\end{tabular}}

\definecolor{DarkYellow}{RGB}{218, 165, 33}
\definecolor{DarkGreen}{RGB}{85, 168, 104}

\newcommand{\quotes}[1]{``#1''}
\newcommand{\gray}[1]{\textcolor{tablegray}{#1}}

\newcommand{\rbt}[1]{\textcolor{blue}{#1}}

\usepackage[boxruled,linesnumbered]{algorithm2e} % algoruled, noend, rightnl
\SetKwInput{KwInput}{Input}
\SetKwInput{KwOutput}{Output} 


\newcommand{\todo}[1]{\colorbox{blue!15}{[todo]: #1}}

\usepackage{booktabs, multirow} % for table borders and merged ranges
\usepackage{makecell}
\usepackage{tabu}
\usepackage{soul}
\newcommand{\ulcolor}[2][Red]{\setulcolor{#1}\ul{#2}}

% \usepackage{caption} % table caption width

% \usepackage{picins}
% \usepackage{natbib}
% \usepackage{subfig}
\usepackage{caption}
\captionsetup[table]{skip=0pt}
% \usepackage{capt-of}
% \usepackage{wrapfig}
\input{lib/insbox}
% this only works when it has text both before
% and after {wrapfigure}
% \begin{wrapfigure}[8]{R}{0.5\textwidth} % the 10 is height. 
% \centering
% \vspace*{-2em} % the starting position
% \begin{minipage}{\linewidth}
% \begin{listing}[H]
%     \python{pseudocode/main.py}
%     \caption{Captions}
%     \label{code}
% \end{listing}
% \end{minipage}
% \end{wrapfigure}


% \newcommand{\mname}{FSDN\:}
\newcommand{\mname}{DE-ViT\:}




==> backup/backup.iclr2024/2.abstract.tex <==



\begin{abstract}


Few-shot object detection aims at detecting novel categories given a few example images. Recent methods focus on finetuning-based strategies to learn features representing novel classes, whose complicated procedures prohibit a wider application. 
In this paper, we introduce DE-ViT, a few-shot object detector without the need for finetuning.
We transform the multi-class classification into multiple binary classifications, so a binary classifier can be trained and used for all classes without finetuning. We propose a novel propagation-based localization mechanism upon frozen DINOv2. 
We evaluate \mname on few-shot, and one-shot object detection benchmarks with COCO and LVIS. For COCO, \mname surpasses the few-shot SoTA by 15 mAP on 10-shot and 7.2 mAP on 30-shot and one-shot SoTA by 2.8 AP50. For LVIS, \mname outperforms few-shot SoTA by 20 box APr. When compared to open-vocabulary detectors, \mname outperforms the COCO SoTA by 6.9 AP50 and achieves 50 AP50 in novel classes, and surpasses LVIS SoTA by 1.5 mask APr and reaches 34.3 mask APr.
% TODO
\keywords{First keyword \and Second keyword \and Third keyword}
% \ifarxiv
% Code is available at \texttt{\href{https://github.com/mlzxy/devit}{https://github.com/mlzxy/devit}}.
% \else
% %
% \fi


\end{abstract}

==> backup/backup.iclr2024/3.introduction.tex <==
\section{Introduction}

 Object recognition and localization are two of the core tasks in computer vision. \emph{Few-shot object detection} provides a promising paradigm for generic object detector by representing novel categories with a set of support images \cite{antonelli2022few}. However, despite the promising practicality in principle, there still exist fundamental limitations in previous work on few-shot object detection. First, most recent few-shot methods rely on finetuning to adapt to novel classes ~\cite{kohler2023few}, a complicated and tedious procedure that restricts the practical use of these methods~\cite{zhao2022semantic}. Second, the accuracy of existing few-shot methods does not keep up with other alternative solutions. Specifically, few-shot detectors fall behind open-vocabulary zero-shot detectors, especially in challenging datasets such as COCO and LVIS~\cite{ma2023digeo, cora2023}. 

 % with the rapid development of vision-language models~\cite{radford2021learning}, 


To alleviate the above limitations, we observe that most recent work represents novel categories with features produced from few-shot training~\cite{kohler2023few}. However, without representation learning, few-shot training may not produce strong enough features. This could hinder few-shot performance.
 Motivated by this, we propose to build a few-shot detector on top of DINOv2~\cite{oquab2023dinov2}, a strong pretrained vision model. 
To avoid finetuning over novel classes, we transform the multi-class classification into multiple binary classifications. Thus, a single binary classifier can be trained and used for all classes without any finetuning on novel classes. 
To accurately localize objects from frozen DINOv2 features, 
we design a novel propagation-based mechanism that localizes each object by propagating a region on the similarity map between DINOv2 features and class prototypes.
Prototypes are class representatives built from support image features. 
With these proposed techniques, we introduce \mname, a few-shot object detector that uses example images to detect novel objects without the need for finetuning. The overall architecture is illustrated in Fig.~\ref{fig:overview}. A demonstration of detecting YCB objects is shown in Fig.~\ref{fig:demo}. 


\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth]{assets/demo.new.png}
   \vspace*{-1.5em}
  \caption{
  Demonstration of the proposed method on YCB objects~\cite{calli2015ycb}.
  \mname with ViT-L/14 is used for prediction. Note that our model is trained on only the
base categories of LVIS. Example images of YCB objects are provided only during inference to represent novel categories.
}
  \label{fig:demo}
\end{figure}

We evaluate \mname on few-shot, and one-shot object detection benchmarks with COCO~\cite{lin2014microsoft} and LVIS~\cite{gupta2019lvis} datasets. Our method establishes new state-of-the-art (SoTA) results on all benchmarks. For COCO,  \mname surpasses the few-shot SoTA LVC~\cite{kaul2022label} by 15 mAP on 10-shot and 7.2 mAP on 30-shot and one-shot SoTA BHRL~\cite{yang2022balanced} by 2.8 AP50. For LVIS, which has been regarded as a highly challenging dataset for few-shot object detection~\cite{wang2020frustratingly},  \mname outperforms the SoTA DiGeo~\cite{ma2023digeo} by 20 box APr. 
When compared to open-vocabulary detectors, DE-ViT outperforms the COCO SoTA CORA\textsuperscript{+}~\cite{cora2023} by 6.9 AP50 and reaches 50 AP50 and LVIS SoTA Ro-ViT~\cite{rovit2023} by 1.5 mask APr, reaching 34.3 mask AP in novel categories.
Notably,  our method only trains on the corresponding dataset, i.e., COCO or LVIS, without leveraging extra datasets for training, or distillation. Our contributions are summarized as follows: (1)  To the best of our knowledge, we are the first to incorporate DINOv2 into solving the few-shot object detection problem. (2) Built upon the techniques motivated above, we introduce DE-ViT, which detects novel objects without any finetuning. (3) We demonstrate that \mname establishes state-of-the-art performance over few-shot and one-shot benchmarks on COCO and LVIS, and outperforms open-vocabulary detectors as well.

% We propose to build a few-shot detector on top of DINOv2, rather than learning feature extractors through few-shot training.

% o realize the generalization ability of DINOv2, ,  We achieve this by transforming multi-class classification into multiple binary classification and propose a novel propagation-based localization method that produces refined boxes from similarity maps. 

\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth]{assets/main-pipeline.drawio.svg.pdf}
  \vspace*{-1.5em}
  \caption{Overview of the proposed method. 
Our approach uses DINOv2 ViT to encode the image into a feature map, from which proposal features are extracted using ROIAlign. Proposals are generated via an off-the-shelf RPN. 
Prototype projection transforms proposal features into similarity maps based on prototypes derived from ViT features of support images.
Multi-class classification of proposals is recast as a series of one-vs-rest binary classification tasks
 without the need for costly per-class inference. 
Refined localization is accomplished by our novel region propagation module. 
  Both classification and refined localization rely exclusively on the computed similarity maps. }
  \label{fig:overview}
\end{figure}




==> backup/backup.iclr2024/4.related_work.tex <==
% \vspace*{-0.5em}
\section{Related work}

% due to the inadequate utilization of
% support data
% \cite{michaelis2018one, hsieh2019one, chen2021adaptive, zhao2022semantic, yang2022balanced}. 

\noindent\textbf{Few-shot Object Detection (FSOD)} aims at detecting objects of novel classes 
by utilizing a few support images from novel classes as training samples \cite{kohler2023few}. Existing approaches 
can be broadly classified into finetuning-based \cite{wang2020frustratingly, fan2021generalized, sun2021fsce, xiao2022few, guirguis2023niff} and meta-learning-based strategies \cite{yan2019meta, kang2019few, fan2020few}. Finetuning-based methods, despite their prevalence, suffer from a large accuracy gap 
between the base and novel classes, as well as practical limitations due to redundant multi-stage  procedures \cite{zhao2022semantic}. Meta-learning methods avoid finetuning by online adaptation, but exhibit inferior accuracy~\cite{kohler2023few}. 
One-shot Object Detection (OSOD) is an extreme case of FSOD with only one exemplar per novel class and simplifies the setting to single-class detection without finetuning~\cite{yang2022balanced}. Prior approaches primarily focus on designing interaction mechanisms of dense spatial features between support and target images 
\cite{antonelli2022few}. 
However, the OSOD formulation restricts the use of additional support and requires a separate inference per class. 
Compared with existing work, 
our method does not use finetuning or per-class inference and only utilizes class-level prototypes without dense feature interactions while outperforming SoTA methods in both few-shot and one-shot settings.



\noindent\textbf{Open-Vocabulary Object Detection (OVD)} aims at detecting objects of novel classes with only their category names and without support images \cite{zareian2021open, yu2023convolutions}. However, despite this more challenging zero-shot setting, with the recent advances in vision-language models~\cite{radford2021learning},  open-vocabulary detectors outperform few-shot ones in COCO and LVIS~\cite{ma2023digeo, cora2023}. Our few-shot detector outperforms the SoTAs on both few-shot and open-vocabulary, which has not been achieved before by existing few-shot work. 


==> backup/backup.iclr2024/5.method.tex <==
\section{Method}
\label{sec:method}

The major challenge in both FSOD is to generalize to classes that are unseen during training. However, despite numerous attempts to this issue, \emph{e.g.}, margin-based regularization~\cite{ma2023digeo}, there persists a considerable accuracy gap between base and novel classes.
This disparity indicates that a network trained with base classes would inevitably fixate on patterns that are only present among a few base classes, which does not align with the objective of detecting arbitrary classes.

To prevent overfitting base class patterns, we propose to use the maps of similarities between the features and prototypes as the detector input. Thus, the network can only make decisions upon relevant information projected by the class representative features. Specifically, let $\mathbf{f} \in \mathbb{R}^{H\times W \times D}$ be the features of an image where $D$ represents the channel dimension and $(H, W)$ represent spatial dimensions, let $\mathbf{p} \in \mathbb{R}^{(C+B)\times D}$ be the prototypes where $C$ is the number of classes and $B$ is the number of class-agnostic background prototypes. Similarity map $\mathbf{s} \in \mathbb{R}^{H\times W \times (C+B)}$ is calculated using Eq.~\ref{eq:similarity-map}. This procedure is referred to in Fig.~\ref{fig:method-class} as prototype projection. 

\vspace*{-1em}

\begin{equation}
\label{eq:similarity-map}
    \mathbf{s} =  \mathbf{f}  \cdot \mathbf{p}^{\top} 
\end{equation}

We adopt a standard two-stage object detection framework, \eg, Mask R-CNN~\cite{he2017mask}, which detects objects through RPN and RCNN stages. Existing literature has demonstrated that class-agnostic RPN proposals generalize well to novel classes \cite{vild2021}. We use off-the-shelf RPNs to propose object regions and extract proposal features from DINOv2 ViT backbones. 
Similarity maps are computed between proposal features and prototypes, which are then 
fed to our architectures for classification and refined localization.
Prototypes are constructed offline from support images with the procedures detailed in Sec.~\ref{sec:method-proto}. 
The ViT backbones, prototypes, and resulting the similarity maps are kept frozen during detector training. 



\subsection{Classification with an Unknown Number of Classes}
\label{sec:method-cls}


Unlike supervised learning, the number of classes in FSOD is indeterminate. The common strategy in FSOD is to extend the final linear layer with finetuning. In contrast with these existing approaches, we transform the multi-classification of $C$ classes into $C$ one-vs-rest binary classification tasks. In doing so, a single binary classifier could be trained and used for all classes without finetuning. However, applying a binary classifier for multi-class classification requires separate inference for each class~\cite{ovdetr2022}. To avoid the costly per-class inference, we apply a class preselection to only predict the probabilities for a small selection of classes.
%%%%%%
Let $\bar{\mathbf{f}} =  \frac{\sum_{i,j=1}^{H,W} \mathbf{f}_{ij}}{H W}  \in \mathbb{R}^D$ be the average feature of a proposal. The class pre-selection procedure returns the top-$K$ mostly likely classes $\mathcal{C}_K = \text{top\_indices}_K(\mathbf{h})$, where $\mathbf{h} \in \mathbb{R}^C$ is the dot-product similarity between $\bar{\mathbf{f}}$ and class prototypes, defined as $\mathbf{h} =\bar{\mathbf{f}} \cdot \mathbf{p}^{\top}$. 
Our method only predicts the probabilities for $\mathcal{C}_K$ and sets the others to 0. As shown in Sec.~\ref{sec:exp-analysis}, our method surpasses SoTA even when $K=3$ on both COCO (80 classes) and LVIS (1203 classes), eliminating the need for costly per-class inference.

% The average feature $\bar{\mathbf{f}}$ is only used to select top classes $\mathcal{C}_K$.

\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth]{assets/preselection+reorder+resample.drawio.svg.pdf}
  \vspace*{-1em}
  \caption{Overview of our classification architecture. Class pre-selection chooses the top-$K$ classes based on the dot product similarity between the average feature of each proposal and class-level prototypes. The probability of each selected class $c_k$ is 
 predicted through a binary classification network, shared by all the classes, in a one-vs-rest manner. The input to this classification network is the similarity map that results from the prototype projection, after rearranging it for each class.}
  \label{fig:method-class}
\end{figure}


For each class $c_k$ in $\mathcal{C}_K$, the similarity map $\mathbf{s} \in \mathbb{R}^{H\times W \times (C+B)}$ (computed in Eq.~\ref{eq:similarity-map}) is rearranged into a class-specific map $\mathbf{s}_{c_k} \in \mathbb{R}^{H\times W \times (1+T+B)}$, as shown in Eq.~\ref{eq:class-specific-sim-map}, where $[C] \backslash c_k$ is defined as $\{1, .., c_k - 1, c_k + 1, ..., C\}$.

\vspace*{-0.5em}

\begin{equation}
    \mathbf{s}_{c_k} = \text{concat}(\mathbf{s}[:,:,c_k], F_{\text{rearrange}}(\mathbf{s}_{[C] \backslash c_k}),\mathbf{s}[:, :, C:C+B]) 
    \label{eq:class-specific-sim-map}
\end{equation}

where $\mathbf{s}_{[C]\backslash c_k} = \text{concat}(\mathbf{s}[:,:,:c_k-1], \mathbf{s}[:,:,c_k+1:])$, and $F_{\text{rearrange}}(\mathbf{x})$ is defined in Eq.~\ref{eq:class-rearrange}. $T$ is a constant hyper-parameter. In Eq.~\ref{eq:class-specific-sim-map}, $\mathbf{s}[:,:,c_k]$, $\mathbf{s}_{[C] \backslash c_k}$, and $\mathbf{s}[:, :, C:C+B]$ represent the similarity map for the current class $c_k$, other classes $[C] \backslash c_k$, and the background, correspondingly.
\vspace*{-1em}

\begin{equation}
      F_{\text{rearrange}}(\mathbf{x}) = \begin{cases} \text{upsample}(\text{sort}(\mathbf{x}), T) & \text{if } T \ge C-1 \\ \text{sort}(\mathbf{x})[:, :, :T] & \text{otherwise} \end{cases}
    \label{eq:class-rearrange}
\end{equation}

\vspace*{-0.5em}

However, it is difficult to input $\mathbf{s}_{[C] \backslash c_k}$ directly to network due to the lack of inherent order in classes and the non-determinate nature of the number of classes in the few-shot setting.  For the first issue, we decide to use magnitude order by sorting $\mathbf{s}_{[C]\backslash c_k}$ along the channel dimension, as in Eq.~\ref{eq:class-rearrange}. For the second issue, we standardize the input size by either keeping the similarity of the top $T$ classes or linearly upsampling the similarity map of all $C-1$ classes to $T$. In doing so, $\mathbf{s}_{[C] \backslash c_k}$ is transformed from $H\times W \times (C-1)$ into a fixed size $H\times W\times T$. Note that the listed functions, \emph{i.e.},  $\text{sort}$, $\text{concat}$ and $\text{upsample}$, are applied along the channel dimension, and $\text{sort}$ works in descending order. 
% 
Finally, the class-specific similarity map $\mathbf{s}_{c_k}$ is given as input to a binary classification network that returns the probability for $c_k$. 
The overall classification architecture is illustrated in Fig.~\ref{fig:method-class}.

\subsection{Localization with Region Propagation.}
\label{sec:method-loc}

% to refine the localization of proposal bounding boxes.

Despite their rich semantics information, ViT features lack the coordinates information required for bounding box regression. As shown in Sec.~\ref{sec:exp-ablation}, naively applying a conventional regression on ViT features yields poor localization results. 
A natural solution is to learn this localization capability by finetuning the ViT backbone during detector training. Similar strategies have demonstrated success in OVD for vision-language backbones, \eg, CLIP \cite{regionclip2022}.
However, we observed that finetuning results in an accuracy collapse on novel classes when text embeddings are replaced with prototypes, which indicates a loss of generalization power. While this phenomenon is intriguing, the practical question is how to produce accurate localization using frozen visual features. 

%  and could potentially extend to vision-only backbones

\vspace*{-0.125em}

\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth]{assets/region-propagation.drawio.svg.pdf}
  \vspace*{-1.75em}
  \caption{Overview of our refined localization architecture. Proposal expansion enlarges each proposal by a fixed ratio to cover more object area. The spatial relationship between the original and expanded proposal is described via a heatmap. The segmentation network navigates the initial heatmap toward accurate object regions. The propagated heatmap is converted into bounding box coordinates through our spatial integral layer. }
  \label{fig:method-localization}
\end{figure}

\vspace*{-0.125em}

%  need to be improved
Our intuition is that only proposals that overlap with objects are important because others would be rejected by the classification network. If we expand such proposals, they would possibly cover the entire region of underlying objects. 
Therefore, original proposals can be refined by predicting object regions within the expanded proposals. We model this procedure as propagating original proposals to object areas in the form of heatmaps. 
The heatmaps can be projected into box coordinates through integral over spatial dimensions. 
The overall refined localization architecture is illustrated in Fig.~\ref{fig:method-localization}.


As shown in Fig.~\ref{fig:method-localization}, the propagation procedure is implemented through binary segmentation. We convert groundtruth bounding boxes to heatmaps that we use to train this segmentation network. Inspired by unsupervised keypoint estimation, particularly the works of IMM~\cite{jakab2018unsupervised} and Transporter~\cite{kulkarni2019unsupervised}, we devise a spatial integral layer to project the propagated heatmap to box. The idea is to learn a transformation that translates the heatmap to a box $(c^{\text{rel}}_w, c^{\text{rel}}_h, w^{\text{rel}}, h^{\text{rel}}) \in [0, 1]^4$ in coordinates that are relative to the expanded proposal. Relative coordinates can be simply mapped back to absolute coordinates. 
%
Let $\mathbf{g} \in \mathbb{R}^{H \times W}$ denote the logits of the propagated heatmap, the relative box $(c^{\text{rel}}_w, c^{\text{rel}}_h, w^{\text{rel}}, h^{\text{rel}})$ can be estimated by our spatial integral layer as explained in Eq.~\ref{eq:spatial-int} and \ref{eq:spatial-int2}. An illustrative example of our spatial integral layer can be found in Figure~\ref{fig:spatial-int}.

\vspace*{-1em}

\begin{equation}
(c^{\text{rel}}_w, c^{\text{rel}}_h) = \sum_{i,j=1}^{H, W} \left(\frac{i}{H}, \frac{j}{W}\right) * \text{softmax}(\mathbf{g})_{ij}
   \label{eq:spatial-int} 
\end{equation}

\vspace{-1em}

\begin{equation}
(w^{\text{rel}}, h^{\text{rel}}) = \left( \sum_{i=1}^{H} \sum_{j=1}^{W}\frac{\sigma(\mathbf{g})_{(i)j}}{W} \mathbf{\theta^w}_i,\,\, \sum_{j=1}^{W} \sum_{i=1}^{H}\frac{\sigma(\mathbf{g})_{i(j)}}{H} \mathbf{\theta^h}_j  \right) 
\label{eq:spatial-int2}    
\end{equation}

\vspace{-0.5em}

\vspace*{2em}
\InsertBoxR{0}{
\begin{minipage}{0.4\textwidth}
  \centering
  \includegraphics[width=\linewidth]{assets/spatial-integral.drawio.svg.pdf}
  \vspace{-1.5em}
  \captionof{figure}{\footnotesize To compute the bounding box of the triangle object from the binary mask, the maximum row and column sum can be used as the box width and height.}
  \label{fig:spatial-int}
\end{minipage}
}[5]

To motivate Eq.~\ref{eq:spatial-int} and \ref{eq:spatial-int2}, consider the toy example of converting a binary mask to a bounding box in Fig.~\ref{fig:spatial-int}. 
A reasonable approach is to compute the mask center as the bounding box center and pick the maximum row and column sum as width and height.
Following the same spirit, we compute the expected position under the spatial distribution $\text{softmax}(\textbf{g})$ as the bounding box center. We compute the row and column sums of sigmoid activation as $\sum_{j=1}^W  \sigma(\textbf{g})_{ij}$ and $\sum_{i=1}^H  \sigma(\textbf{g})_{ij}$. Instead of picking the maximum, we aggregate all row or column sums in terms of magnitude. The rationale of this aggregation is that a larger estimation is more likely to over-cover the entire object and a small estimation may produce a box too tight. The aggregation is done by sorting the estimation and then weighted averaging.
This explains the use of order statistics notation $(i)$ and $(j)$, and $\mathbf{\theta^h} \in \mathbb{R}^{W}, \mathbf{\theta^w} \in \mathbb{R}^{H}$  are learnable aggregation weights.
Finally, the relative coordinates are mapped to absolute ones by Eq.~\ref{eq:map-to-abs}, where $(c^{\text{exp}}_w, c^{\text{exp}}_h, w^{\text{exp}} , h^{\text{exp}})$ is the expanded proposal.

\vspace*{-1em}

\begin{align}
\begin{split}
&(w^{\text{out}}, h^{\text{out}}) = (w^{\text{exp}} \, w^{\text{rel}}, h^{\text{exp}} \, h^{\text{rel}}) \\
&(c^{\text{out}}_w, c^{\text{out}}_h) = (c_w^{\text{exp}} - 0.5 w^{\text{exp}}, c_h^{\text{exp}} - 0.5 h^{\text{exp}}) + (c^{\text{rel}}_w \, w^{\text{exp}}, c^{\text{rel}}_h \, h^{\text{exp}})
   \label{eq:map-to-abs} 
\end{split}
\end{align}

% \vspace*{em}

During training, we use groundtruth bounding boxes as regression targets for the output of spatial integral layer. Similar to our classification pipeline, the localization procedure is applied for each class in $\mathcal{C}_K$ to produce class-specific boxes. For each class $c_k$, only the similarity map of $c_k$ and the background will be selected as input. We omit this detail in Fig.~\ref{fig:method-localization} for visual clarity.

\subsection{Building Prototypes}
\label{sec:method-proto}

Similar to the pioneering FSOD work Meta R-CNN~\cite{yan2019meta}, our method represents classes with prototype vectors constructed from visual features of given support images. The main difference in building prototypes is that we use the features from pretrained DINOv2 while Meta R-CNN uses region features from its detection network.
%
Fig.~\ref{fig:build-prototype} shows the process of building instance-level prototypes. 
For each object instance, its prototype is computed as the mean ViT feature from corresponding regions defined by either a segmentation mask or bounding box.
Next, class-representing prototypes are obtained by averaging the cluster centroids of instance-level prototypes for each class.
%
We use the online clustering method proposed by SwAV~\cite{caron2020unsupervised}, though we find that simply averaging all instance prototypes for each class achieves similar results. Prototypes of base classes are built from the entire training set instead of support images, which are used only for novel classes.

\vspace*{1em}

\InsertBoxR{0}{{
\begin{minipage}{0.5\linewidth}
  \vspace{-0.5em}
  \includegraphics[width=\linewidth]{assets/instance-prototype.drawio.svg.pdf}
  \vspace*{-2em}
  \captionsetup{font=footnotesize}
  \captionof{figure}{Overview of building instance prototypes.}
  \label{fig:build-prototype}
\end{minipage}
}}[3]

To build background prototypes, we start from the obervation that backgrounds typically share similar visual attributes, such as uniform motion, smooth texture, static color tone, \emph{etc}. 
Moreover, the ability to capture and thereby separate background from foreground is crucial. 
Because of the lack of visual diversity yet the importance of background semantics, 
we use masks for a fixed list of background classes, \emph{e.g.}, sky, wall, road, and apply a similar prototype-building procedure. 
The idea of using background information for few-shot performance is similarly explored in IPRNet~\cite{okazawa2022interclass}.
In contrast with class-level prototypes that change upon class configurations, background prototypes are always fixed as a part of the network's parameters. All the prototypes are built offline and frozen during training and inference.


% 

==> backup/backup.iclr2024/6.experiment.tex <==

\section{Experiments}
\label{sec:exp}

\begin{table}\centering
\caption{Results on COCO 2014 few-shot benchmark. Our method outperforms existing work in detecting novel classes by a significant margin and does not require finetuning on novel classes.}
\label{tab:coco-fewshot}
\resizebox{\linewidth}{!}{
\scriptsize
\begin{tabu}{rc|c|cccc|cccc}\toprule
\rowfont{\normalsize} \multicolumn{2}{c|}{\multirow{2}{*}{Method}} & \multirow{2}{*}{\footnotesize \vspace{0.4em} Finetune} &\multicolumn{4}{c}{\normalfont 10-shot} &\multicolumn{4}{c}{\normalfont 30-shot} \\\cmidrule{4-11}
\rowfont{\footnotesize} &  & {\footnotesize on Novel} &bAP &nAP &nAP50 &nAP75 &bAP &nAP &nAP50 &nAP75 \\\midrule
\multicolumn{2}{l|}{FSRW \cite{kang2019few}} & \xmark &- &5.6 &12.3 &4.6 &- &9.1 &19 &7.6 \\
\multicolumn{2}{l|}{Meta R-CNN \cite{yan2019meta}} & \xmark  &5.2 &6.1 &19.1 &6.6 &7.1 &9.9 &25.3 &10.8 \\
\multicolumn{2}{l|}{TFA \cite{wang2020frustratingly}} & \cmark  &33.9 &10 &19.2 &9.2 &34.5 &13.5 &24.9 &13.2 \\
\multicolumn{2}{l|}{Multi-Relation Det \cite{fan2020few}} & \xmark  &- &16.6 &31.3 &16.1 &- &- &- &- \\
\multicolumn{2}{l|}{FSCE \cite{sun2021fsce}} & \cmark &- &11.9 &- &10.5 &- &16.4 &- &16.2 \\
\multicolumn{2}{l|}{Retentive RCNN \cite{fan2021generalized}} & \cmark &39.2 &10.5 &19.5 &9.3 &39.3 &13.8 &22.9 &13.8 \\
\multicolumn{2}{l|}{HeteroGraph \cite{han2021query}}& \cmark &- &11.6 &23.9 &9.8 &- &16.5 &31.9 &15.5 \\
\multicolumn{2}{l|}{FsDetView \cite{xiao2022few}}& \cmark &6.4 &7.6 &- &- &9.3 &12 &- &- \\
\multicolumn{2}{l|}{Meta Faster RCNN \cite{han2022meta}}& \cmark &- &12.7 &25.7 &10.8 &- &16.6 &31.8 &15.8 \\
\multicolumn{2}{l|}{LVC \cite{kaul2022label}}& \cmark &28.7 &19 &34.1 &19 &34.8 &26.8 &45.8 &27.5 \\
\multicolumn{2}{l|}{CrossTransformer \cite{han2022few}}& \cmark &- &17.1 &30.2 &17 &- &21.4 &35.5 &22.1 \\
\multicolumn{2}{l|}{NIFF \cite{guirguis2023niff}}& \cmark &39 &18.8 &- &- &39 &20.9 &- &- \\
\multicolumn{2}{l|}{DiGeo \cite{ma2023digeo}}& \cmark &39.2 &10.3 &18.7 &9.9 &39.4 &14.2 &26.2 &14.8 \\\midrule
\multirow{3}{*}{\mname (Ours)} &ViT-S/14 & \xmark  &24 &\textbf{27.1} &\textbf{43.1} &\textbf{28.5} &24.2 &\textbf{26.9} &\textbf{43.1} &\textbf{28.4} \\
&ViT-B/14 & \xmark  &28.3 &\textbf{33.2} &\textbf{51.4} &\textbf{35.5} &28.5 &\textbf{33.4} &\textbf{51.4} &\textbf{35.7} \\
&ViT-L/14 & \xmark  &29.4 &\textbf{34.0} &\textbf{53.0} &\textbf{37.0} &29.5 &\textbf{34.0} &\textbf{52.9} &\textbf{37.2} \\
\bottomrule
\end{tabu}
}
% \vspace{-1em}
\end{table}


We comprehensively evaluate our method on few-shot, one-shot benchmarks, and compare it to open-vocabulary detectors. 
Furthermore, we compare the efficiency of our method against SoTA solutions, study few-shot performance on different numbers of shots, and provide qualitative results. 
We conduct ablations to show that a naive combination of DINOv2 and Meta R-CNN leads to unsatisfying results, and every proposed component is important to the performance of our method.

\noindent\textbf{Evaluation Metrics and Datasets.} Few-shot, one-shot, and open-vocabulary evaluations split classes into base and novel classes. Base classes are seen during training and novel classes are unseen. The performance on novel classes is more important. For COCO, nAP, nAP50, and nAP75 represent mAP, AP50, and AP75 in novel classes. bAP and bAP50 represent mAP and AP50 in base classes. One-shot evaluation conventionally divides 80 classes of COCO into four even partitions, and alternatively takes three as base classes and one partition as novel classes~\cite{michaelis2018one}. There are 4 base/novel splits in total, named Split-1/2/3/4. For LVIS, APr, APc, and APf represent AP on rare, common, and frequent categories. Rare categories are used as novel classes. Metrics on LVIS are computed separated on bounding boxes, \emph{e.g.}, box APr, or instance segmentation masks, \emph{e.g.}, mask APr. We evaluate our method on COCO 2014, COCO 2017~\cite{lin2014microsoft}, and LVIS-v1~\cite{gupta2019lvis}. We follow the conventional base/novel classes split with existing work~\cite{wang2020frustratingly, yang2022balanced, regionclip2022}. Note that the few-shot benchmark uses COCO 2014, while the one-shot and open-vocabulary benchmarks use COCO 2017.


\noindent\textbf{Model Specifications.} We use DINOv2~\cite{oquab2023dinov2} ViT as the feature extractor, and report results in ViT-S/B/L (small, base, large) model sizes.
We train a ResNet50 RPN separately for each dataset using only base classes and use 1000 proposals in all settings. We detail the design of binary classification and segmentation networks in Sec.~\ref{apn:more-impl-details}. 
Class prototypes are built upon instance masks in support images unless specified.
We use the same support images as sampled by previous work~\cite{wang2020frustratingly, yang2022balanced} for few-shot and one-shot settings. When comparing with open-vocabulary detectors, we sample 30 instances per class (30-shot) using the protocol of \cite{wang2020frustratingly} for the support set. 
Background prototypes are extracted from background classes, \emph{e.g.}, sky, road, by the semantic masks in COCOStuff~\cite{cocostuff}.


\subsection{Main Results}
\label{sec:exp-main-results}


Tab.~\ref{tab:coco-fewshot} shows our results on few-shot COCO benchmark. \mname outperforms the previous SoTA LVC by a significant margin (+15 nAP on 10-shot, +7.2 nAP on 30-shot). It is worth noting that LVC requires over ten stages for self-training and pseudo-labeling procedures~\cite{kaul2022label}. A pretrained model for LVC has never been released. Other recent few-shot works also include multiple pretraining and finetuning stages~\cite{han2022meta, han2022few}. Our proposed method DE-ViT can be trained in a single stage and used on novel objects directly without any fine-tuning. The difference between 30-shot (nAP50=52.9) and 10-shot (nAP50=53.0) is smaller than 0.1\% and could be interpreted as statistically insignificant. 

LVIS has been regarded as a highly challenging dataset in FSOD~\cite{wang2020frustratingly} and only DiGeo~\cite{ma2023digeo} reports few-shot results on LVIS v1. Tab.~\ref{tab:lvis-fewshot} shows that our method outperforms DiGeo in all metrics and a significant boost in the accuracy of detecting novel objects (+20 box APr).



Tab.~\ref{tab:coco-oneshot} shows our results on one-shot COCO. \mname outperforms the previous SoTA BHRL by 6 bAP50 and 2.8 nAP50. 
One-shot methods follow a single-class detection setting. We adapt DE-ViT by detecting each class separately during evaluation. It is worth noting that our proposed DE-ViT can perform both one-shot and few-shot detection using the same model.
OWL-ViT~\cite{owlvit2023} also reports one-shot results on COCO. However, OWL-ViT's results are obtained with an ensemble of open-vocabulary and one-shot pipelines without providing implementation or isolated measurements. Therefore, we only compare against OWL-ViT with our few-shot setting in Tab.~\ref{tab:ovd}. 


% COCO, one-shot
\begin{table}\centering
\caption{Results on COCO 2017 one-shot benchmark. \mname outperforms existing work and is not limited to single class detection and single support image as other one-shot methods.}\label{tab:coco-oneshot}
\resizebox{\linewidth}{!}{
\scriptsize
\begin{tabu}{lrrrrrrrrrrr}\toprule
\rowfont{\normalsize} &\multicolumn{5}{c}{bAP50} &\multicolumn{5}{c}{nAP50} \\\cmidrule{2-11}
&Split-1 &Split-2 &Split-3 &Split-4 &Avg &Split-1 &Split-2 &Split-3 &Split-4 &Avg \\\midrule
SiamMask \cite{michaelis2018one} &38.9 &37.1 &37.8 &36.6 &37.6 &15.3 &17.6 &17.4 &17 &16.8 \\
CoAE \cite{hsieh2019one} &42.2 &40.2 &39.9 &41.3 &40.9 &23.4 &23.6 &20.5 &20.4 &22 \\
AIT \cite{chen2021adaptive} &50.1 &47.2 &45.8 &46.9 &47.5 &26 &26.4 &22.3 &22.6 &24.3 \\
SaFT \cite{zhao2022semantic} &49.2 &47.2 &47.9 &49 &48.3 &27.8 &27.6 &21 &23 &24.9 \\
BHRL \cite{yang2022balanced} &56 &52.1 &52.6 &53.4 &53.6 &26.1 &29 &22.7 &24.5 &25.6 \\
\midrule \mname  (Ours, ViT-L/14) &\textbf{59.4} &\textbf{57.0} &\textbf{61.3} &\textbf{60.7} &\textbf{59.6} &27.4 &\textbf{33.2} &\textbf{27.1} &\textbf{26.1} &\textbf{28.4} \\
\bottomrule
\end{tabu}}
% \vspace{-1.5em}
\end{table}

\begin{minipage}{0.6\textwidth}
\captionof{table}{Performance comparison with existing few-shot object methods on LVIS dataset. We report box AP as evaluation metrics.}
\label{tab:lvis-fewshot}
\footnotesize
\begin{tabu}{lr|cccc}\toprule
\rowfont{\normalsize} \multicolumn{2}{c}{Method} &APr &APc &APf &AP \\\midrule
\multicolumn{2}{c}{DiGeo \cite{ma2023digeo}} &16.6 &22.8 &28 &24.4 \\\midrule
\multirow{3}{*}{\mname (Ours)} &ViT-S/14 &\textbf{23.4} &22.8 &22.5 &22.8 \\
&ViT-B/14 &\textbf{26.8} &\textbf{26.5} &25.3 &\textbf{26} \\
&ViT-L/14 &\textbf{33.6} &\textbf{30.1} &\textbf{30.7} &\textbf{30.9} \\
\bottomrule
\end{tabu}
\end{minipage}
\hfill
\begin{minipage}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{assets/coco14.pdf}
    \vspace*{-2.5em}
    \captionof{figure}{Performance of our method and few-shot SoTA at different shots.}
    \label{fig:shots}
\end{minipage}


\begin{table}
\centering
\caption{Comparison to open-vocabulary detectors on LVIS and COCO 2017. $\dagger$: Customized pretrained model is used instead of public models. \quotes{-} denotes result that is not reported. The best and second-best are bolded and underlined.}
\label{tab:ovd}
\footnotesize
\begin{tabular}{c|c|c|cc|c}\toprule
\multirow{2}{*}{Method} &\multirow{2}{*}{Backbone} &Use Extra & \multicolumn{2}{c}{LVIS} & COCO  \\
& &Training Set &mask APr &box APr & nAP50 \\\midrule
% OVR-CNN \cite{zareian2021open} &RN50 &\cmark  & - & - & 22.8 \\
ViLD \cite{vild2021} &EffNet-B7 &\xmark &26.3 &27 &27.6 \\
RegionCLIP \cite{regionclip2022} &RN50x4 &\cmark &- &22  & 39.3\\
OV-DETR \cite{ovdetr2022} &ViT-B/32 &\xmark &- &17.4 & 29.4 \\
Detic \cite{detic2022} &RN50 &\cmark &17.8 &- & 27.8 \\
OWL-ViT \cite{owlvit2023} &ViT-L/14\textsuperscript{$\dagger$} &\xmark &- &25.6 & - \\
OWL-ViT \cite{owlvit2023} &ViT-L/14\textsuperscript{$\dagger$} &\cmark &- &\underline{31.2} & - \\
CORA\textsuperscript{+} \cite{cora2023} & RN50x4 &	\cmark &- &28.1  & 43.1 \\
Ro-ViT \cite{rovit2023} &ViT-L/14\textsuperscript{$\dagger$} &\xmark &31.4 &- & 33 \\
Co-Det \cite{ma2024codet} & Swin-B  &\cmark & 29.4 & - & 30.6 \\
F-VLM \cite{rovit2023} & RN50x64 &\xmark & \underline{32.8} &- & 28.0 \\
\midrule \multicolumn{1}{c|}{\multirow{3}{*}{\mname 
 (Ours)}} &ViT-S/14 &\xmark & 24.2 &  23.4 & 39.5 \\
  &ViT-B/14 &\xmark & 28.5 & 26.8  & \underline{45.4} \\
  &ViT-L/14 &\xmark &  \textbf{34.3} &\textbf{33.6} & \textbf{50} \\
\bottomrule
\end{tabular}
\end{table}
% \begin{table}
% \centering
% \caption{Comparison to open-vocabulary detectors on LVIS and COCO 2017. $\dagger$: Customized pretrained model is used instead of public models. \quotes{-} denotes result that is not reported. The best and second-best are bolded and underlined.}
% \label{tab:ovd}
% \footnotesize
% \begin{tabular}{c|c|c|cc|c}\toprule
% \multirow{2}{*}{Method} &\multirow{2}{*}{Backbone} &Use Extra & \multicolumn{2}{c}{LVIS} & COCO  \\
% & &Training Set &mask APr &box APr & nAP50 \\\midrule
% % OVR-CNN \cite{zareian2021open} &RN50 &\cmark  & - & - & 22.8 \\
% ViLD \cite{vild2021} &EffNet-B7 &\xmark &26.3 &27 &27.6 \\
% RegionCLIP \cite{regionclip2022} &RN50x4 &\cmark &- &22  & 39.3\\
% OV-DETR \cite{ovdetr2022} &ViT-B/32 &\xmark &- &17.4 & 29.4 \\
% Detic \cite{detic2022} &RN50 &\cmark &17.8 &- & 27.8 \\
% OWL-ViT \cite{owlvit2023} &ViT-L/14\textsuperscript{$\dagger$} &\xmark &- &25.6 & - \\
% OWL-ViT \cite{owlvit2023} &ViT-L/14\textsuperscript{$\dagger$} &\cmark &- &\underline{31.2} & - \\
% CORA\textsuperscript{+} \cite{cora2023} & RN50x4 &	\cmark &- &28.1  & 43.1 \\
% Ro-ViT \cite{rovit2023} &ViT-L/14\textsuperscript{$\dagger$} &\xmark &31.4 &- & 33 \\
% Co-Det \cite{ma2024codet} & EVA02-L\textsuperscript{$\dagger$}  &\cmark & \textbf{37} & - & 30.6 \\
% F-VLM \cite{rovit2023} & RN50x64 &\xmark &32.8 &- & 28.0 \\
% \midrule \multicolumn{1}{c|}{\multirow{3}{*}{\mname 
%  (Ours)}} &ViT-S/14 &\xmark & 24.2 &  23.4 & 39.5 \\
%   &ViT-B/14 &\xmark & 28.5 & 26.8  & \underline{45.4} \\
%   &ViT-L/14 &\xmark &  \underline{34.3} &\textbf{33.6} & \textbf{50} \\
% \bottomrule
% \end{tabular}
% \end{table}


We compare DE-ViT against open-vocabulary detectors in Tab.~\ref{tab:ovd}. \mname outperforms the previous SoTA CORA\textsuperscript{+} by 6.9 AP50. Our method only trains on COCO while CORA\textsuperscript{+} uses ImageNet-21K~\cite{krizhevsky2012imagenet} and COCO Captions~\cite{cococap} as additional training data. When only using COCO, \mname outperforms CORA by 8.3 AP50. 
In LVIS, \mname outperforms the previous SoTA on mask APr (+1.5 over F-VLM) and box APr (+2.4 over OWL-ViT).
We follow a multi-scale instance segmentation head design, as detailed in  Sec.~\ref{apn:more-impl-details}. 

We observe a high variance in the performance of OVD detectors in Tab.~\ref{tab:ovd}. F-VLM achieves a mask APr of  32.8 on LVIS but only has 28 nAP50 on COCO. While CORA\textsuperscript{+} has 43.1 nAP50 on COCO but only a box APr of 28.1 on LVIS. On the contrary, our DE-ViT outperforms existing solutions on both LVIS (34.3 mask APr) and COCO (50 nAP50). We acknowledge the task setting difference of this comparison. Our few-shot method \mname has access to support images that language-based detectors do not. However, we emphasize that \mname outperforms the SoTAs on both few-shot and open-vocabulary, which has not been achieved before by existing few-shot work.



\subsection{Analysis}
\label{sec:exp-analysis}

\begin{minipage}{0.46\textwidth}
\centering
\captionof{table}{\footnotesize  Inference time comparison on COCO with existing few-shot methods.}\label{tab:speed-few-shot}
\scriptsize
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}\toprule
&Backbone & Secs/Img &nAP50 \\\midrule
{\tiny Meta FasterRCNN~\cite{han2022meta}} &RN101 &0.61 &31.8 \\
{\tiny CrossTransformer~\cite{han2022few}} &Custom &3 &35.8 \\
DE-ViT (Ours) &ViT-S &\textbf{0.25} &\textbf{42.7} \\
\bottomrule
\end{tabular}
}
\end{minipage}
\hfill
\begin{minipage}{0.55\textwidth}
\centering
\captionof{table}{\footnotesize Comparison of training epoch and parameter size to other  detectors trained on LVIS.}\label{tab:params-train}
\scriptsize
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccc}\toprule
 &  \mcell{Total \\ Params}  & \mcell{Trained \\ Params} &Epochs &APr \\\midrule
OWL-ViT~{\tiny \cite{owlvit2023}}  &433M &433M &1800 &31.2 \\
F-VLM~{\tiny\cite{kuo2022f}} &445M &25M &118 &32.8 \\
DE-ViT (Ours) &350M &\textbf{23M} &\textbf{14.4} &\textbf{34.3} \\
\bottomrule
\end{tabular}}
\end{minipage}

\noindent\textbf{Efficiency.} We compare the inference time of \mname against recent few-shot works in Tab.~\ref{tab:speed-few-shot}. 
Tab.~\ref{tab:speed-few-shot} shows that \mname has the smallest inference time, while having better accuracy.
We compare the parameter sizes and training epochs of detectors trained on the large-scale dataset LVIS in Tab.~\ref{tab:params-train}. 
Tab.~\ref{tab:params-train} shows that \mname only has 23M trainable parameters, and is trained orders of magnitude faster than F-VLM~\cite{kuo2022f} and OWL-ViT~\cite{owlvit2023}.
The inference time of all methods is measured under the same machine.
We conduct inference time comparisons under different values of $K$ and detail the efficiency discussion in Sec.~\ref{apn:exp}.



\noindent\textbf{More shots.}  To study the model performance with different numbers of shots, we plot the nAP50 with different shots in Fig.~\ref{fig:shots} and Fig.~\ref{fig:shots17}  for COCO 2014 and COCO 2017, correspondingly.
It can be seen that performance generally increases with the number of shots, and there exists an inflection point after which more samples do not help.
 The inflection point is located around 50 to 75 shots for COCO 2017 and 6 shots for COCO 2014. We detail the shot sampling setup in Sec.~\ref{apn:more-shots}.


\noindent\textbf{Qualitative Results.} We provide qualitative comparisons of our proposed DE-ViT and Meta Faster RCNN in Fig.~\ref{fig:coco-14-q} and Fig.~\ref{fig:coco-14-more-q}. DE-ViT detects more novel objects while having fewer false positives. 
Note that Meta Faster RCNN can only detect novel objects after finetuning, while DE-ViT can detect both base and novel classes without finetuning. We provide more visualizations in 
 Fig.~\ref{fig:lvis-q} and \ref{fig:coco-17-more-q}.


\subsection{Ablation Study}
\label{sec:exp-ablation}

    
\begin{table}
\begin{minipage}{0.62\textwidth}
\begin{minipage}{\textwidth}
\caption{Ablation studies on the classification architecture. }
\label{tab:ablation-cls}
\scriptsize
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccc|cccc}\toprule
Conventional &Prototype &Background &Class  &\multicolumn{2}{c}{Novel} &\multicolumn{2}{c}{Base} \\
Prototype Head & Projection & Tokens &  Rearrange &nAP50 &nAP75 &bAP50 &bAP75 \\\midrule
\cmark & & & &4.5 &2.2 &48.9 &22.5 \\
&\cmark & & &26.2 &9.7 &29.3 &12 \\
&\cmark &\cmark & &38.4 &23 &43.4 &26.8 \\
&\cmark &\cmark &\cmark &39.5 &24.1 &42.3 &25.9 \\
\bottomrule
\end{tabular} }
\vspace{0.5em}
\end{minipage}
\begin{minipage}{\textwidth}
\caption{Ablation studies on the propagation localization.}
\label{tab:ablation-reg}
\scriptsize
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccc|cccc}\toprule
Conventional &Expanded & Spatial Integral &\multicolumn{2}{c}{Novel} &\multicolumn{2}{c}{Base} \\
REG Head &Proposal & over Heatmap &nAP50 &nAP75 &bAP50 &bAP75 \\\midrule
\cmark & & &37.7 &14.6 &46.5 &23.9 \\
\cmark &\cmark & &35.6 &12.5 &41.3 &19.8 \\
&\cmark &\cmark &39.5 &24.1 &42.3 &25.9 \\
\bottomrule
\end{tabular}}
\end{minipage}
\end{minipage}
\hfill
\begin{minipage}{0.36\textwidth}
\vspace{-1em}
\centering
    \rotatebox{90}{\hspace{2em} \footnotesize Ours}
      \includegraphics[width=0.65\textwidth]{assets/qualitative/coco14/478874.jpg}
    
     \rotatebox{90}{\hspace{-0.5em}\footnotesize Meta Faster RCNN}
       \includegraphics[width=0.65\textwidth]{assets/qualitative/coco14/478874.ref.jpg}

    \vspace{0.7em}
    \captionof{figure}{\footnotesize Qualitative comparison against Meta Faster RCNN. More visualizations can be found in Fig.~\ref{fig:bad-case}, \ref{fig:lvis-q}, ~\ref{fig:coco-14-more-q}, and \ref{fig:coco-17-more-q}.}
    \label{fig:coco-14-q}
\end{minipage}
\end{table}
% \quotes{blue} and \quotes{yellow} denote base and novel classes. 


\noindent\textbf{Naive Combination of DINOv2 and Meta RCNN.} Our initial attempt is to integrate DINOv2 into the framework of Meta RCNN~\cite{yan2019meta}, a classic prototype-based few-shot detector. Specifically, we build prototypes from DINOv2 features and use the prototype features as the weights for the last linear layer of the classification network. The only difference between the above procedure and Meta RCNN is how to build prototypes. We use DINOv2 features and Meta RCNN uses average features of the output from ROIAlign in a detection network. It is worth noting that this procedure is also similar to RegionCLIP which uses text embedding features to compose the weights of the last classification linear layer. As shown in Tab.~\ref{tab:ablation-cls}, this conventional prototype head design produces almost no few-shot ability (4.5 nAP50). This suggests that 
combining DINOv2 and prototype-based few-shot detectors is not trivial.


\noindent\textbf{Classification.} We examine the component effects for classification in Tab.~\ref{tab:ablation-cls}. Tab.~\ref{tab:ablation-cls} shows that the model completely overfits base classes without our proposed components. By learning from similarity maps from prototype projection, general detection ability emerges, and then improves after adding the background prototypes and the class rearrange module. Results in Tab.~\ref{tab:ablation-cls}, \ref{tab:ablation-reg} and \ref{tab:ablation-bbox} are obtained with ViT-S/14.

\noindent\textbf{Refined Localization.} We study the impacts of propagation-based localization in Tab.~\ref{tab:ablation-reg}. For the conventional REG head, we use a CNN with both features and similarity maps as input. Novel classes 
 have poor localization (14.6 AP75) without our proposed architecture, and simply expanding proposals even lowers the performance. The localization accuracy jumps to 24.1 AP75 when our proposed spatial integral layer is used to produce bounding boxes from the propagated heatmaps.

\noindent\textbf{Using Boxes or Masks to Build Prototypes.}  In Tab.~\ref{tab:ablation-bbox}, we study the effects of annotation types, \emph{i.e.}, bounding boxes or masks, in constructing prototypes. We observe that using bounding boxes to build prototypes yields almost indistinguishable performance compared to using instance masks at even 5-shot in COCO 2014. Our main results use prototypes built from instance masks. 







==> backup/backup.iclr2024/7.discussion.tex <==
\section{Conclusion}
\label{sec:conclusion}


In this work, we propose DE-ViT, a few-shot detector that uses example images to detect novel classes without any finetuning. We demonstrate that DE-ViT establishes new state-of-the-art in few-shot and one-shot benchmarks. DE-ViT also outperforms open-vocabulary detectors, which has not been achieved before by existing few-shot work. DE-ViT detects objects using only frozen DINOv2 features. Therefore, it is straightforward to integrate DE-ViT with backbones other than DINOv2. One of the limitations is that our current architecture is a mix of ViT and RCNN, while a full transformer network can clearly be more scalable and unlock more possible abilities and integrations to other modalities. Another limitation is that our current model relies on an external region proposal network (RPN). It is possible to train an RPN on top of frozen DINOv2 with some engineering efforts. We hope that our work will be useful in downstream tasks such as robotic manipulation, and help other researchers develop better methods for few-shot object detection. 






==> backup/backup.iclr2024/8.foot.tex <==
% placeholder









==> backup/main.tex <==
\input{root}
% \input{supplementary}

==> backup/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> backup/method.tex <==
\section{Method}
\label{sec:method}

\vspace{-0.5em}


\subsection{Problem Formulation}

We use $\mathcal{C}$ to denote the set of classes. In few-shot object detection (FSOD), $\mathcal{C}$ is composed of a set of base classes, denoted by $\mathcal{C}_{base}$, and a set of novel classes, denoted by $\mathcal{C}_{novel}$. Thus, $\mathcal{C} = \mathcal{C}_{base} \cup \mathcal{C}_{novel}$ and $\mathcal{C}_{base} \cap \mathcal{C}_{novel} = \varnothing$. During training, a large number of  examples are provided for the base classes. During testing, only $k$ labeled samples are provided for each novel class. The samples for novel classes are  referred to as {\it support images}. The goal is to leverage the training data of $\mathcal{C}_{base}$ to learn a detector that can detect objects of $\mathcal{C}_{novel}$ given the $k$-shot support images.



\subsection{Region Propagation Network}

\begin{figure}[ht]
  \centering
  \vspace*{-1em}
  \includegraphics[width=\linewidth]{assets/corl/main-rpropnet.jpg}
  \vspace*{-1.75em}
  \caption{\small Overview of the proposed method. Given a proposal box of a query image, we extract the initial mask region (\ulcolor[yellow]{yellow}) and expand the proposal by a constant ratio. Next, the region within the expanded proposal is gradually propagated and refined to fit the object area through a sequence of propagation layers. Each propagation layer accepts previous regions and features as input while returning updated features and region as outputs. The final predicted region is transformed to bounding-box coordinates through a learnable spatial integral layer, as detailed in Sec.~\ref{sec:spatial-integral}. 
  The predicted region also serves as spatial attention to average features along height and width. The averaged features are then mapped to class scores. 
  The projected features are the dot products between the ViT features of a query image and class prototypes, as detailed in Sec.~\ref{sec:feat-sub-proj}.
  }
  % \vspace*{-2em}
  \label{fig:pipeline}
  \vspace{-1em}
\end{figure}



Despite having rich semantics information, pretrained ViT features lack the coordinates information required for bounding box regression. As shown in Appendix~\ref{sec:analysis}, naively applying a conventional regression on ViT features yields poor localization results. 
A natural solution is to learn this localization capability by finetuning the ViT backbone during the training of the detector with the base classes. 
However, we observed that finetuning results in completely overfitting the base classes and in an accuracy collapse on novel classes. This was observed when integrating DINOv2 ViT into the framework of Meta RCNN~\cite{yan2019meta}, a standard prototype-based FSOD, as shown in Appendix~\ref{sec:analysis}. 
This suggests that  harnessing the generalization power of strong ViT backbones for FSOD is non-trivial. The question here is how to produce accurate localization with pretrained ViT features. 



% Our intuition is that only proposals that significantly overlap with objects are important to the localization accuracy because others are likely to be background.
% If we iteratively expand such proposals, they would eventually cover the entire region of underlying objects. 
% Therefore, objects can be localized by predicting a mask among the expanded proposals instead of performing a bounding box regression. We therefore present a region propagation network that propagates proposal regions to object regions.  The output regions are then transformed into box coordinates through an integral over spatial dimensions. 

Given an object proposal, we use a region propagation network that gradually propagates the proposal region to accurately cover and fit the object by refining an object mask. Unlike bounding-box regression, mask prediction localizes objects without coordinate outputs. The propagated region is then transformed into a bounding box through a learnable spatial integral layer. We use an off-the-shelf region proposal network (RPN) to generate the initial region proposals, as class-agnostic proposals are shown to generalize well to novel classes~\cite{vild2021}. Each proposal is expanded by a fixed ratio in order to delimit the propagation boundaries. The overall framework is shown in Fig.~\ref{fig:pipeline}.




\vspace{0.5em}\noindent\textbf{Propagation Layer.} We propose the region {\it Propagation Layer} (PL), a new type of network module designed for object detection. PL serves as the central building block of our method. An example is shown in Fig.~\ref{fig:region-prop-show}. The $t$-th PL block takes all previous regions $r_{0:t-1} \in \mathbb{R}^{t\times K\times K}$ and the previous PL block features $h_{t-1} \in \mathbb{R}^{S\times K \times K}$ as input, where $t$ denotes the number of PL blocks, $S$ denotes the number of feature channels, and $K$ denotes the feature spatial size. The $t$-th PL block outputs the updated region $r_t \in \mathbb{R}^{1\times K\times K}$, features $h_t\in \mathbb{R}^{S\times K \times K}$, bounding box $b_t \in \mathbb{R}^4$, and class score $c_t \in \mathbb{R}$. 
Each PL block works as a small detection network and can be stacked to improve accuracy. The update rule is explained in Eq.~\ref{eq:PL} and illustrated in the third part of Fig.~\ref{fig:pipeline}. 


\vspace{-0.5em}
\begin{equation}
\begin{aligned}
h_t = f_{\text{update}, t}(\operatorname{concat}(r_{0:t-1}, h_{t-1});\theta),\,\, h_{t,region} = f_{\text{region}, t}(h_t;\theta)\\
r_t = \sigma(h_{t, region}),\,\, b_t = f_{\text{integral}, t}(h_{t,region};\theta) \\
c_t = f_{\text{class}, t}(\text{\scriptsize WeightedAvgPool}(h_t, r_t); \theta)
\end{aligned}
\label{eq:PL}
\end{equation}

In Eq.~\ref{eq:PL}, $f_{\text{update}, t}$ denotes the conv-bn-relu block with $S$ output channels that updates the hidden features, and $\text{concat}$ denotes channel-wise concatenation. $f_{\text{region}, t}$ denotes the conv block with single channel output that predicts the output region logits $h_{t,region} \in \mathbb{R}^{1\times K\times K}$. $\sigma$ denotes the sigmoid function. $f_{\text{integral}, t}$ denotes the spatial integral layer detailed in Sec.~\ref{sec:spatial-integral}. 
$h_t$ is aggregated over spatial dimensions to $\text{\footnotesize WeightedAvgPool}(h_t, r_t) \in \mathbb{R}^{S\times1\times1}$ with weights $r_t$. $f_{\text{class}, t}$ denotes the linear block that maps $\text{\footnotesize WeightedAvgPool}(h_t, r_t)$ to class scores. $\theta$ denotes network parameters. 
%%
During training, we use focal loss and L1 regression loss for the output class score $c_t$ and bounding box $b_t$. For the output region $r_t$, we apply BCE loss and Dice loss~\cite{sudre2017generalised}. The region labels during training are generated by the ground-truth object region within the expanded proposals.




\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{assets/corl/region_vis.pdf}
  \vspace*{-1.5em}
  \caption{\small Region propagation on class \enquote{fridge}. The proposal, expanded proposals, and final predicted boxes are colored in \ulcolor[maize]{transparent yellow}, \ulcolor[lemon]{yellow}, and \ulcolor[green]{green}, respectively. The three propagated regions (from left to right) are sampled from the output of the first three PL blocks in ascending order.}
  \label{fig:region-prop-show}
  \vspace{-2em}
\end{figure}

\subsection{Learnable Spatial Integral}
\label{sec:spatial-integral}

Converting masks to bounding boxes is a widely-used transformation in instance segmentation networks~\cite{ren2023detrex} as a post-processing step. The standard solution is to find the top-left and bottom-right foreground pixels and use their positions as the bounding box coordinates~\cite{torchvision2016}. However, this approach has major limitations. 
Firstly, this mask-to-box conversion assumes the availability of ground-truth instance masks, which are much more expensive to obtain than bounding boxes~\cite{lin2014microsoft}. 
%Therefore, a mask-to-box transformation independent of instance masks is more generally useful. 
Moreover, this approach is non-differentiable and is also prone to outliers. Therefore, the question is how to accurately derive bounding boxes from the region-based localization results using a learnable and differentiable function.

\vspace{0.5em}\noindent Let $b^{\text{out}} = (c_{w}^{\text{out}}, c_{h}^{\text{out}}, w^{\text{out}}, h^{\text{out}})$ denote the output bounding box, where $c_{w}^{\text{out}} \in [0, W], w^{\text{out}} \in [0, W]$ and $c_{h}^{\text{out}} \in [0, H], h^{\text{out}} \in [0, H]$. Instead of predicting $b^\text{out}$ directly, we propose to first predict a relative bounding box $b^{\text{rel}} = (c_{w}^{\text{rel}}, c_{h}^{\text{rel}}, w^{\text{rel}}, h^{\text{rel}}) \in [0, 1]^4$, that can be transformed to $b^{\text{out}}$ according to Eq.~\ref{eq:map-to-abs},
\begin{align}
\begin{split}
&(w^{\text{out}}, h^{\text{out}}) = (w^{\text{exp}} \, w^{\text{rel}}, h^{\text{exp}} \, h^{\text{rel}}), \\
&(c^{\text{out}}_w, c^{\text{out}}_h) = (c_w^{\text{exp}} - 0.5 w^{\text{exp}}, c_h^{\text{exp}} - 0.5 h^{\text{exp}}) + (c^{\text{rel}}_w \, w^{\text{exp}}, c^{\text{rel}}_h \, h^{\text{exp}}),
   \label{eq:map-to-abs} 
\end{split}
\end{align}

\vspace{0.25em}

where $b^{\text{exp}} = (c_{w}^{\text{exp}}, c_{h}^{\text{exp}}, w^{\text{exp}}, h^{\text{exp}})$ denotes the expanded proposal. Thus, $b^{\text{rel}}$ is a normalized bounding box relative to $b^{\text{exp}}$. Let $h_{region} \in \mathbb{R}^{K\times K}$ denote the output region logits, where we skip the notation of $t$-th block and the channel of $1$ for simplicity.
Our spatial integral layer $f_{\text{integral}}$ estimates $b^\text{rel}$  with Eq.~\ref{eq:spatial-int} and \ref{eq:spatial-int2}. An illustrative example is given in Fig.~\ref{fig:spatial-int}.

\begin{table}
\begin{minipage}{.4\textwidth}
\centering
\includegraphics[width=\linewidth]{assets/eccv/main-spatial-integral.jpeg}
\captionof{figure}{\footnotesize The max row sum and column sum are used as the box width and height of the triangular object.}\label{fig:spatial-int}
\end{minipage}
\begin{minipage}{.6\textwidth}
\begin{equation}
(c^{\text{rel}}_w, c^{\text{rel}}_h) = \scaleto{\sum_{i,j=1}^{K, K}}{2.5em} \scaleto{\left(\frac{i}{K}, \frac{j}{K}\right)}{2em} * \text{\footnotesize softmax}(h_{region})_{ij}
   \label{eq:spatial-int} 
\end{equation}
\begin{equation}
\begin{aligned}
w^{\text{rel}}= \sum_{i=1}^{K} \sum_{j=1}^{K}  \frac{\sigma(h_{region})_{(i)j}}{K} \mathbf{\theta^w}_i \\
h^{\text{rel}} = \sum_{j=1}^{K} \sum_{i=1}^{K} 
 \frac{\sigma(h_{region})_{i(j)}}{K} \mathbf{\theta^h}_j 
\label{eq:spatial-int2}    
\end{aligned}
\end{equation}
\end{minipage}
\vspace{-2em}
\end{table}
% \vspace{0.5em}

To motivate Eq.~\ref{eq:spatial-int} and \ref{eq:spatial-int2}, consider the toy example of converting a binary triangle mask to a bounding box in Fig.~\ref{fig:spatial-int}. 
A reasonable approach is to compute the mask center as the bounding box center and use the max row sum and column sum as width and height.
Inspired by this insight, we compute the expected position of the spatial distribution $\text{softmax}(h_{region})$ as the center of $b^{\text{rel}}$ in Eq.~\ref{eq:spatial-int}. We compute the row and column sums of the output region as $\sum_{j=1}^K  \sigma(h_{region})_{ij}$ and $\sum_{i=1}^K  \sigma(h_{region})_{ij}$ in Eq.~\ref{eq:spatial-int2}. Instead of picking the maximum, we apply a soft aggregation to average all row or column sums in terms of magnitude rank. The aggregation is done by sorting the row and column sums, and then computing the weighted average. This explains the use of order statistics notation $(i)$ and $(j)$. Parameters $\mathbf{\theta^h} \in \mathbb{R}^{K}, \mathbf{\theta^w} \in \mathbb{R}^{K}$  are learnable aggregation weights. 




\begin{table}[t]\centering
\caption{\small Results on COCO 2014 few-shot benchmark. Our method outperforms existing work in detecting novel classes by a significant margin. Results surpassing the SoTA are indicated in bold.}
\label{tab:coco-fewshot}
\resizebox{\linewidth}{!}{
\scriptsize
\begin{tabu}{rc|c|cccc|cccc}\toprule
\rowfont{\scriptsize} \multicolumn{2}{c|}{\multirow{2}{*}{Method}} & \multirow{2}{*}{\scriptsize \vspace{0.4em} Requires} &\multicolumn{4}{c}{\scriptsize 10-shot} &\multicolumn{4}{c}{\scriptsize 30-shot} \\\cmidrule{4-11}
\rowfont{\scriptsize} &  & {\scriptsize Finetune} &bAP &nAP &nAP50 &nAP75 &bAP &nAP &nAP50 &nAP75 \\\midrule
\multicolumn{2}{l|}{FSRW \cite{kang2019few}} & \xmark &- &5.6 &12.3 &4.6 &- &9.1 &19 &7.6 \\
\multicolumn{2}{l|}{Meta R-CNN \cite{yan2019meta}} & \xmark  &5.2 &6.1 &19.1 &6.6 &7.1 &9.9 &25.3 &10.8 \\
\multicolumn{2}{l|}{TFA \cite{wang2020frustratingly}} & \cmark  &33.9 &10 &19.2 &9.2 &34.5 &13.5 &24.9 &13.2 \\
\multicolumn{2}{l|}{Multi-Relation Det \cite{fan2020few}} & \xmark  &- &16.6 &31.3 &16.1 &- &- &- &- \\
\multicolumn{2}{l|}{FSCE \cite{sun2021fsce}} & \cmark &- &11.9 &- &10.5 &- &16.4 &- &16.2 \\
\multicolumn{2}{l|}{Retentive RCNN \cite{fan2021generalized}} & \cmark &39.2 &10.5 &19.5 &9.3 &39.3 &13.8 &22.9 &13.8 \\
\multicolumn{2}{l|}{HeteroGraph \cite{han2021query}}& \cmark &- &11.6 &23.9 &9.8 &- &16.5 &31.9 &15.5 \\
\multicolumn{2}{l|}{FsDetView \cite{xiao2022few}}& \cmark &6.4 &7.6 &- &- &9.3 &12 &- &- \\
\multicolumn{2}{l|}{Meta Faster RCNN \cite{han2022meta}}& \cmark &- &12.7 &25.7 &10.8 &- &16.6 &31.8 &15.8 \\
\multicolumn{2}{l|}{LVC \cite{kaul2022label}}& \cmark &28.7 &19 &34.1 &19 &34.8 &26.8 &45.8 &27.5 \\
\multicolumn{2}{l|}{CrossTransformer \cite{han2022few}}& \cmark &- &17.1 &30.2 &17 &- &21.4 &35.5 &22.1 \\
\multicolumn{2}{l|}{NIFF \cite{guirguis2023niff}}& \cmark &39 &18.8 &- &- &39 &20.9 &- &- \\
\multicolumn{2}{l|}{DiGeo \cite{ma2023digeo}}& \cmark &39.2 &10.3 &18.7 &9.9 &39.4 &14.2 &26.2 &14.8 \\\midrule
\multirow{3}{*}{\mcell{\mname \\ (Ours)}} &ViT-S/14 & \xmark  &24 &\textbf{27.1} &\textbf{43.1} &\textbf{28.4} &24.2 &\textbf{26.9} & 43.1&\textbf{28.5} \\
&ViT-B/14 & \xmark  &28.3 &\textbf{33.2} &\textbf{51.4} &\textbf{35.5} &28.5 &\textbf{33.4} &\textbf{51.4} &\textbf{35.7} \\
&ViT-L/14 & \xmark  &29.4 &\textbf{34.0} &\textbf{52.9} &\textbf{37.0} &29.5 &\textbf{34.0} &\textbf{53.0} &\textbf{37.2} \\
\bottomrule
\end{tabu}
}
% \vspace{-1em}
\end{table}



\subsection{Feature Subspace Projection}
\label{sec:feat-sub-proj}

The main challenge of FSOD is to generalize to novel classes that are unseen during training. However, despite numerous attempts to solving this problem, by using margin-based regularization for example~\cite{ma2023digeo}, there persists a considerable accuracy gap between base and novel classes~\cite{antonelli2022few}. This disparity indicates that a network trained with base classes would inevitably overfit on patterns that are only present among the base classes. A classic technique to reduce overfitting consists in representing data in a low-rank subspace~\cite{SCHITTENKOPF1997505}. We explore in this work the construction of a subspace of pre-trained ViT features that reduces the accuracy gap between base and novel classes. 

% Inspired by the principle component analysis (PCA), 
% , which does not align to detect arbitrary novel classes

Prototypes are class representatives built from support images. Given the support images of each class, we compute the ViT features, crop the features with object bounding boxes and use the average feature as the class prototype~\cite{yan2019meta}. 
%%
Let $p_\mathcal{C} \in \mathbb{R}^{|\mathcal{C}|\times D}$ denote the prototypes of classes from set $\mathcal{C}$, where $D$ denotes the channel dimension. Let $h_{vit} \in \mathbb{R}^{D\times H\times W}$ denote the ViT features of the query image. We assume that both prototypes and features are normalized to unit length at the channel dimension. Then $p_\mathcal{C} \cdot h_{vit} \in \mathbb{R}^{|\mathcal{C}|\times H\times W}$ can be interpreted as a subspace projection with  $p_\mathcal{C}$ being the basis. However, this subspace construction has two limitations. Firstly, only using prototypes of classes set $\mathcal{C}$ can be too limited to sufficiently capture the feature information. Secondly, a permutation of $\mathcal{C}$ creates a different but equivalent subspace, yet designing permutation-invariant networks is a highly challenging problem~\cite{hensel2021survey}. For the first limitation, we introduce a  set  $\mathcal{B}$ of background classes, $\mathcal{B}\cap\mathcal{C} = \varnothing$, with  $p_\mathcal{B} \in \mathbb{R}^{|\mathcal{B}|\times D}$ being the prototypes of $\mathcal{B}$, to preserve more information from $h_{vit}$. For the second limitation, we propose to build a separate subspace for each class $c \in \mathcal{C}$, and reorder other classes $\mathcal{C}\setminus c$ to resolve permutation ambiguity. The feature subspace projection is explained in Eq.~\ref{eq:subspace} and illustrated in Fig.~\ref{fig:pipeline}.

\vspace{-1em}

\begin{align}
h_{subspace,c} = \operatorname{concat}(p_c \cdot h_{vit}, \operatorname{channel-reorder}(p_{\mathcal{C}\setminus c} \cdot h_{vit}), p_{\mathcal{B}} \cdot h_{vit}) 
\label{eq:subspace}
\end{align}

In Eq.~\ref{eq:subspace}, $h_{subspace,c} \in \mathbb{R}^{S\times H \times W}$ denotes the subspace feature for class $c$, and function \rbt{$\operatorname{channel-reorder}$ sorts the $|\mathcal{C}|-1$ channels of input tensor $p_{\mathcal{C}\setminus c} \cdot h_{vit} \in \mathbb{R}^{(|\mathcal{C}|-1) \times H \times W}$ by magnitude at each spatial location, and then linearly interpolates the tensor to a pre-defined size $(S - 1 - |\mathcal{B}|) \times H \times W$, where $S$ is a constant hyperparameter.} In practice, we use example images of non-object stuff classes, \textit{e.g.}, sky, road, floor, to construct $\mathcal{B}$. 
As shown in Appendix~\ref{sec:analysis}, feature subspace projection significantly reduces the accuracy gap between base and novel classes. On the other hand, creating a subspace for each class $c \in \mathcal{C}$ introduces costly per-class inference. However, the per-class inference cost can be reduced by finding the top $T$ most likely classes with a lightweight prototype classifier~\cite{yan2019meta} and only performing inference for these $T$ classes.
As shown in Appendix~\ref{sec:analysis}, 
our method achieves a faster inference speed and surpasses SoTA when $T = 3$.




